Domain-Independent Deception: A New Taxonomy and Linguistic Analysis

Internet-based economies and societies are drowning in deceptive attacks. These attacks take many forms, such as fake news, phishing, and job scams, which we call ``domains of deception.'' Machine-learning and natural-language-processing researchers have been attempting to ameliorate this precarious situation by designing domain-specific detectors. Only a few recent works have considered domain-independent deception. We collect these disparate threads of research and investigate domain-independent deception. First, we provide a new computational definition of deception and break down deception into a new taxonomy. Then, we analyze the debate on linguistic cues for deception and supply guidelines for systematic reviews. Finally, we investigate common linguistic features and give evidence for knowledge transfer across different forms of deception.

==> Hide/bios.tex <==

\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,trim=10cm 10cm 10cm 10cm,clip]{profile/rv-acm-pic-top-white.jpg}}]{Rakesh M. Verma} (M 2013) is a Professor of Computer Science at the University of Houston (UH) where he leads the Reasoning and Data Analytics for Security (ReDAS) group. 
\end{IEEEbiography}
\section{Conclusion} \label{sec-concl}
We have provided a new definition and a taxonomy for deception to clarify the scope of deception and give impetus to domain-independent deception detection.  We gave sound desiderata for systematic review and meta-analysis to help researchers conduct high quality literature analyses and devise new domain-independent detection techniques. 
%
We have argued against hasty conclusions regarding linguistic cues for deception detection and especially their generalizability. 
The Critiques~\cite{fitzpatrickBF15,vogler2020using,vrij08} may present a valid point, namely that linguistic cues might not generalize across the broad class of attacks. However, more sweeping statements should be made with caution, as they discourage future domain-independent deception research and evidence suggests they are likely to be at least partly off the mark. 



%We defined what makes a fake news dataset high quality and then conducted a variety of analyses to determine the quality of six datasets. We obtained statistically significant differences between True and False classes for many attributes in very dataset. Some differences were ubiquitous across all datasets. These deserve further analysis because they might indicate universal attributes of fake news, contradicting the hypothesis that deception does not leave a stylistic trace~\cite{grondahlA19}. Other attributes, like cosine similarity and $n$-gram analysis, differ uniquely within classes of individual datasets. This suggests either that:
%\begin{itemize}
 %   \item fake news has obvious, easily detectable differences from real news, or
 %   \item current fake news datasets do not have enough uniformity between classes and variance in instances across all classes.
%\end{itemize}
%We ranked datasets based on the number and size of inter-class differences on our measures (minimal difference, some difference and significant difference). Based on our rankings (Table \ref{rankingstable} \hl{this table has been commented out}), the LIAR dataset has the highest rank and the Kaggle dataset has the lowest  rank amongst the body texts of datasets we analyzed. For headline texts, the two subsets of the FakeNewsNet dataset come out on top and the Kaggle dataset again has the lowest rank.

With all the new developments in machine learning and NLP, research on cues of deception is poised to take off and could result in significant advances.
%Cross-dataset analysis of five different deception datasets and some preliminary multi-domain deep-learning experiments show that there are linguistic features that can be used to build classifiers for more general deception datasets. 
We expect that BERT-based classifiers will perform well on multiple datasets.

\bibliographystyle{plain}
\bibliography{eacl,ref}




%The second paragraph uses the pronoun of the person (he or she) and not the 
%author's last name. It lists military and work experience, including summer 
%and fellowship jobs. Job titles are capitalized. The current job must have a 
%location; previous positions may be listed 
%without one. Information concerning previous publications may be included. 
%Try not to list more than three books or published articles. The format for 
%listing publishers of a book within the biography is: title of book 
%(publisher name, year) similar to a reference. Current and previous research 
%interests end the paragraph. The third paragraph begins with the author's 
%title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter). 
%List any memberships in professional societies other than the IEEE. Finally, 
%list any awards and work for IEEE committees and publications. If a 
%photograph is provided, it should be of good quality, and 
%professional-looking. Following are two examples of an author's biography.
%\end{IEEEbiography}




